Call for Rigor in Reporting Quality of Instruction Tuning Data

Instruction tuning is crucial for adapting large language models (LLMs) to align with user intentions. Numerous studies emphasize the significance of the quality of instruction tuning (IT) data, revealing a strong correlation between IT data quality and the alignment performance of LLMs. In these studies, the quality of IT data is typically assessed by evaluating the performance of LLMs trained with that data. However, we identified a prevalent issue in such practice: hyperparameters for training models are often selected arbitrarily without adequate justification. We observed significant variations in hyperparameters applied across different studies, even when training the same model with the same data. In this study, we demonstrate the potential problems arising from this practice and emphasize the need for careful consideration in verifying data quality. Through our experiments on the quality of LIMA data and a selected set of 1,000 Alpaca data points, we demonstrate that arbitrary hyperparameter decisions can make any arbitrary conclusion.

==> Tables/prevs/tb_lima.tex <==

% \multirow{3}{*}{\textbf{@}}
% \multicolumn{2}{c|}{\textbf{Language}}

\begin{table}[t]
\centering
\resizebox{1.0\linewidth}{!}{
\small
\begin{tabular}{c|cccc}

\toprule[1.5pt]
\textbf{Paper} & \textbf{Epochs} & \textbf{LR} & \textbf{LR Scheduler} & \textbf{Batch} \\ \midrule[1.5pt]

\multicolumn{5}{c}{\textit{Training \textbf{Llama-2-7B} with \textbf{LIMA}}} \\ \midrule[1.5pt]

\citet{DBLP:journals/corr/abs-2407-08995} & 8 & 1e-5 & Cosine & 64 \\
\citet{lima} & 15 (ES) & 1e-5 & Linear & 64 \\
\citet{liu2024selectit} & 3 & 2e-5 & Cosine & 128 \\
\citet{zhao2024long} & 15 & 1e-5 & Linear & 128 \\ 
\citet{ghosh2024closer} & 3 & 5e-5 & - & 32 \\ 
 
\bottomrule[1.5pt]

\end{tabular}
}
\caption{
기존 연구들에서 llama-2-7B language model을 학습하는 데 사용되었던 hyper parameter들. 각 논문들 모두 각자의 hyperparameter를 사용하였으나, 이들을 선택한 rationale가 구체적으로 report되지는 않았다. '-'는 해당 연구들에서 report되지 않은 값을 의미하며, (ES)는 early stopping이 적용된 경우를 의미한다. } \label{tb:lima}
\end{table}


==> Tables/prevs/tb_survey1.tex <==

% \multirow{3}{*}{\textbf{@}}
% \multicolumn{2}{c|}{\textbf{Language}}

\begin{table*}[t]
\centering
% \resizebox{0.48\textwidth}{!}{
\small
\begin{tabular}{c|cccccccc}

\toprule[1.5pt]
\makecell[c]{\textbf{Paper}} & \textbf{\# Data} & \textbf{Epochs} & \textbf{LR} & \textbf{LR Scheduler} & \textbf{Batch} & \textbf{Length} & \textbf{Weight Decay} & \textbf{Warmup Rate} \\ \midrule[1.5pt]

\citet{lima} & 1K & 15 & 1e-5 & Linear & 64 & 2,048 & 0.1 & 0.0 \\ \midrule

\multirow{2}{*}{\citet{zhao2024long}} & 52K & 3 & 2e-5 & Cosine & 128 & 512 & 0.0 & 0.3 \\
& 1K & 15 & 1e-5 & Linear & 128 & 2,048 & 0.1 & 0.0 \\ \midrule

\citet{chen2024alpagasus} & 1K & 3 & 2e-5 & - & 128 & - & - & - \\ \midrule

\citet{xia2024less} & 13K & 4 & 2e-5 & Linear & 128 & - & - & - \\ \midrule

\citet{alpaca} & 52K & 4 & 2e-5 & Cosine & 128 & 512 & 0.0 & 0.03 \\ \midrule

\citet{howfar} & 2.7M & 2 & 2e-5 & Linear & 128 & 2,048 & - & 0.03 \\ \midrule

\citet{lu2024instag} & 6K & 5 & 2e-5 & - & 128 & - & - & - \\ \midrule

% 이 아래로는 mistral임
\citet{liu2024what} & 6K & 5 & 2e-5 & Cosine & 512 & 2,048 & 0.1 & - \\ \midrule

\citet{DBLP:journals/corr/abs-2407-08995} & 1K & 4 & 1e-5 & Cosine & 64 & 4,096 & 0.0 & - \\ \midrule

\multirow{2}{*}{\citet{zhao2024long}} & 52K & 3 & 4e-6 & Cosine & 128 & 512 & 0.0 & 0.3 \\
& 1K & 15 & 2e-6 & Linear & 128 & 2,048 & 0.1 & 0.0 \\ \midrule

\citet{hu2024fine} & 52K & 3 & 2e-5 & Linear & 128 & 2,048 & 0.0 & 0.03 \\ \midrule

\bottomrule[1.5pt]

\end{tabular}
% }
\caption{
기존 연구들에서 llama-2-7B language model을 학습하는 데 사용되었던 hyper parameter들. 각 논문들 모두 각자의 hyperparameter를 사용하였으나, 이들을 선택한 rationale가 구체적으로 report되지는 않았다. Table에서 report하는 연구들은 대부분 Neurips, ICML, ICLR등 notable top-tier conference에 공개된 논문들을 포함하여, 기존 학계들에서 그 영향력을 인정받고 있는 연구들만을 가져왔다. '-'는 해당 연구들에서 report되지 않은 값을 의미한다.} \label{tb:encdec}
\end{table*}


==> Tables/prevs/tb_survey2.tex <==

% \multirow{3}{*}{\textbf{@}}
% \multicolumn{2}{c|}{\textbf{Language}}

\begin{table*}[t]
\centering
\resizebox{0.956\textwidth}{!}{
\small
\begin{tabular}{c|c|cccc}

\toprule[1.5pt]
\textbf{Data} & \textbf{Paper} & \textbf{Epochs} & \textbf{LR} & \textbf{LR Scheduler} & \textbf{Batch} \\ \midrule[1.5pt]

\multicolumn{6}{c}{\textit{Training \textbf{Llama-2-7B}}} \\ \midrule[1.5pt]

\multirow{5}{*}{\makecell[c]{Sampled 1,000 data \\ from Alpaca \\ \cite{alpaca}}} & \citet{du2023mods} & 3 & 2e-5 & Cosine & 128 \\

 & \citet{liu2024selectit} & 3 & 2e-5 & Cosine & 128 \\

 & \citet{mekala2024smaller} & 3 & 2e-5 & Cosine & 128 \\
 & \citet{zhao2024long} & 15 & 1e-5 & Linear & 128 \\ 
 & \citet{yu2024diversify} & 3 & 1e-5 & - & 64 \\
 \midrule

%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \multirow{5}{*}{\makecell[c]{Lima \\ \cite{lima}}} & \citet{DBLP:journals/corr/abs-2407-08995} & 8 & 1e-5 & Cosine & 64 \\
 & \citet{lima} & 15 (ES) & 1e-5 & Linear & 64 \\
 & \citet{liu2024selectit} & 3 & 2e-5 & Cosine & 128 \\
 & \citet{zhao2024long} & 15 & 1e-5 & Linear & 128 \\ 
 & \citet{ghosh2024closer} & 3 & 5e-5 & - & 32 \\ 
 
 \midrule[1.5pt]

 %%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{6}{c}{\textit{Training \textbf{Llama-2-13B} with 1K IT data}} \\ \midrule[1.5pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{5}{*}{\makecell[c]{Sampled 1,000 data \\ from Alpaca \\ \cite{alpaca}}} & \citet{treeinst} & 10 & 1e-4 & - & 16 \\

 & \citet{ghosh2024closer} & 3 & 5e-5 & - & 32 \\ 
 
 & \citet{liu2024selectit} & 3 & 2e-5 & Cosine & 128 \\

 & \citet{mekala2024smaller} & 3 & 2e-5 & Cosine & 128 \\

 & \citet{zhao2024long} & 15 & 1e-5 & Linear & 128 \\ \midrule[1.5pt]
 %%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{6}{c}{\textit{Training \textbf{Mistral 7B}}} \\ \midrule[1.5pt]
 %%%%%%%%%%%%%%%%%%%%%%%%%%%
 \multirow{3}{*}{\makecell[c]{Lima \\ \cite{lima}}} & \citet{DBLP:journals/corr/abs-2407-08995} & 4 & 1e-5 & Cosine & 64 \\
 & \citet{zhao2024long} & 15 & 2e-6 & Linear & 128 \\  
 & \citet{ghosh2024closer} & 3 & 5e-5 & - & 32 \\ \midrule

%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\multirow{3}{*}{\makecell[c]{Sampled 1,000 data \\ from IT Data Mix \\ (wizardlm)}} & \citet{yu2024diversify} & 3 & 1e-5 & - & 64 \\

 & \citet{entropylaw} & 4 & 4e-6 & - & 128 \\

 & \citet{zhao2024long} & 15 & 2e-6 & Linear & 128 \\ \midrule
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\multirow{5}{*}{\makecell[c]{Alpaca \\ (52K)}} & \citet{xiao2024sftmix} & 3 & 2e-6 & Cosine & 32 \\

 & \citet{yu2024diversify} & 3 & 1e-5 & - & 64 \\

 & \citet{fan2024reformatted} & 20 & 6.55e-5 & Cosine & 64 \\

 & \citet{zhao2024long} & 3 & 4e-6 & Cosine & 128 \\ 
 & \citet{ghosh2024closer} & 3 & 5e-5 & - & 32 \\ 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%
  
\bottomrule[1.5pt]

\end{tabular}
}
\caption{
기존 연구들에서 llama-2-7B language model을 학습하는 데 사용되었던 hyper parameter들. 각 논문들 모두 각자의 hyperparameter를 사용하였으나, 이들을 선택한 rationale가 구체적으로 report되지는 않았다. Table에서 report하는 연구들은 대부분 Neurips, ICML, ICLR등 notable top-tier conference에 공개된 논문들을 포함하여, 기존 학계들에서 그 영향력을 인정받고 있는 연구들만을 가져왔다. '-'는 해당 연구들에서 report되지 않은 값을 의미한다.} \label{tb:encdec}
\end{table*}


==> sections/prevs/Section1_241213-1039.tex <==
\section{Introduction}

Large Language Models (LLMs) exhibit remarkable proficiency across a broad spectrum of language understanding and generation tasks. Their adaptability and strong human-interactive capability make them valuable across various fields. Instruction Tuning (IT) is one of the most prevalent methods to attain such human-interactive capability. 
IT involves finetuning LLMs using instruction-response pair data, enabling LLMs to generate appropriate text responses to human instructions.
It facilitates the alignment of models with human preferences and their knowledge base, enabling the generation of desired outputs in response to various instructions \cite{cao2023instruction}.

In implementing IT, data quality is considered a crucial factor. 다량의 IT데이터가 확보되더라도, 그 데이터를 전부 사용하여 학습하는 것보다 그 중 고품질의 IT를 선별하여 학습하는 것이 더욱 높은 alignment성능을 내는 데 더욱 효과적이라는 것은, 여러 연구들을 통해 밝혀진 바 있다. 고품질 데이터를 선별하는 것 이외로도, 고품질 데이터를 만들어서, 기존 데이터보다 더 높은 alignment performance를 내고자 하는 연구들도 현재는 다수 연구되고 있는 바이다.

이러한 연구들을 수행하는 데 있어서는, 구축된 데이터가 고품질이라는 점을 검증할 필요가 있다. 지금까지 거의 모든 연구들에서는, 본인들이 구축한 데이터와 baseline데이터를 LLM에 학습하고, 학습된 모델의 성능을 비교하는 방식의 평가 방법을 적용하였다. 이 경우, 학습된 모델의 성능은 데이터의 품질을 대표한다고 간주된다. These studies mostly  conducted under the assumption that "good data makes a good model." Consequently, most studies aim to demonstrate the quality of the data under evaluation by training such data onto one (possibly several) models and reporting their performance. In this context, "data that makes a good model" is regarded as "good data."

\input{Tables/tb_survey}

이들 대부분은 하나의 실험 세팅을 정의하고, 동일한 실험 세팅 내에서 학습된 모델의 성능을 비교하는 방식을 적용하고 있다. 하지만 우리는, 이러한 연구들에서 검증용 모델 학습을 위한 hyperparameter setting에 대해서 거의 아무런 justification을 이루고 있지 않음을 발견하였다.
Table~\ref{} illustrates the various hyperparameter settings adopted when performing IT using sampled 1K general domain IT data in existing research. As evident, even when training the same model with the same data size, the settings differ across studies.


We argue that caution is required when conducting verification in this manner and reporting the results. As data quality는 indirect measure를 통해 측정되기 때문에, hyperparameter와 같이 모델 성능을 변화시킬 수 있는 요소는, 평가하고자 하는 data quality에 bias를 부여할 수 있다. In particular, we highlight that the reported outcomes can be interpreted differently depending on the arbitrarily chosen hyperparameter settings. 이는 보여주고자 하는 목표에 따라서 이후 심각한 deceit을 발생시킬 위험이 있다.

One might question that coherently applied training setting을 통해 학습했다면, data quality에 대해 robust한 결론을 내릴 수 있는것 아닌가 하며 의문을 가질 수 있다. However, we contend that even with an identical setting, if hyperparameter choices are made arbitrarily, conclusions regarding data quality can also be arbitrarily determined.

As a representative case, we consider two datasets for evaluation: LIMA and Alpaca-longest. In \cite{zhao2024long}, it was reported that a model trained on Alpaca-longest outperformed a model trained on LIMA. We demonstrate how such conclusions can change depending on the hyperparameter selection during the training of the evaluation model, and we draw the community's attention to the ambiguity resulting from these differences.

Finally, we emphasize the necessity of rigorously performing hyperparameter selection when reporting data quality, and we propose a protocol for more robust and rigorous reporting of experimental results.


% LLM은 remarkable proficiency across a broad spectrum of language understanding and generation tasks, adhering to human instructions with effectiveness and safety. 다양한 분야에서 높은 적응성을 보이며 활발하게 사용되고 있다. 
% 이러한 효과를 얻는 데에는, LLM의 high human-interactive performance가 일조한다고 볼 수 있다. 이러한 capability를 얻기 위해 수행되는 Instruction tuning (IT)는 large language model을 human-interative aligning하기 위해 사용되는 가장 prevalent방법 중 한가지이다. 

% 이를 수행함에 있어서 data quality는 매우 중요한 요소로 여겨진다. 최근 LIMA에서는 1천개의 데이터만으로 high alignment performance를 얻을 수 있음을 보여주고 있으며, alpagasus등의 연구에서는, 다량의 데이터를 사용하는 것보다, 좋은 품질의 데이터만을 선별해서 사용하는 것이 higher performance를 위해 필수적인 요소임을 보여주고 있다. 이러한 연구들에 힘입어, 현재 다수의 연구들은 고품질의 instruction tuning data의 선별이라는 주제를 두고 다양한 방법론들을 시도하고 있다. 

% 이러한 연구들은 under the assumption that "good data makes good model"하에 진행된다. In terms of training data, "good data" is defined as a data that makes "good model". 이에, 대부분의 연구들에서는 검증을 목표로 하는 data가 high quality임을 보여주기 위해, 하나의 모델 (possibly several models)을 학습하고, 이들의 성능을 report하는 방법을 사용한다. 이 경우, "data that makes good model" is regarded as "good data". 

% However, as far as we know, 현재 대부분의 연구들은 자체적인 experimental setting을 한가지 정의해두고, 이 세팅 하에 학습된 모델의 성능을 비교하는 방식으로 데이터의 품질을 가늠하고 있다. 이 상황에서 우리가 발견한 것은, 이러한 검증용 모델을 학습하는 데 있어서 세워지는 세팅이, 별다른 rationale 없이 설정되고 있으며, 심지어 서로 다른 연구들간에 통일되어 있지도 않다는 것이다. Table~\ref{}는, 기존 연구들에서 lima데이터를 사용하여 IT를 수행할 때 도입한 hyperparameter setting을 보여준다. 이를 통해 확인할 수 있듯, 동일한 모델, 동일한 데이터로 학습하는 경우에 있어서도, 세팅은 모두 서로 다르다는 것을 확인할 수 있다.

% 우리는 이러한 방식의 검증을 수행하고 결과를 report를 함에 있어서 주의해야 할 필요가 있음을 밝힌다. 특히, 우리는 어떠한 hyperparameter setting을 선택하는지에 따라서 reporting 결과가 다르게 해석될 수 있음을 밝힌다.
% One may wonder that, coherent한 experimental setting을 정의하고 평가용 모델을 학습했다면, data quality에 대해서 robust한 결론을 내릴 수 있는 것이 아닌지 의문을 가질 수 있다. 하지만 아무리 동일한 세팅을 결정한다 하더라도, 우리가 hyperparameter setting을 임의대로 결정한다면, 데이터 품질에 대한 우리의 결론도 우리의 자의적으로 내릴 수 있다고 말할 수 있다. 

% 우리는 대표적으로 Lima데이터와 Alpaca-longest데이터 두가지를 평가 대상으로 삼는다. \cite{zhao2024long}에서 alpaca-longest로 학습한 모델은 lima로 학습한 모델보다 우월한 성능을 보였음이 report된 바 있다. 우리는 평가용 모델 학습을 위한 hyperparameter selection에 따라서, 이러한 결론이 어떻게 바뀔 수 있는지 보고하며, 이러한 차이에 따른 ambiguity에 대한 community의 관심을 환기한다.

% 우리는 최종적으로, 데이터 품질을 report함에 있어서, hyperparameter 결정을 엄밀하게 수행할 필요가 있음을 밝히며, 보다 robust하고 엄밀한 실험 결과 reporting을 위한 protocol에 대해 제안한다. 


% These studies are conducted under the assumption that "good data makes a good model." In terms of training data, "good data" is defined as data that produces a "good model." Consequently, most studies aim to demonstrate the quality of the data under evaluation by training such data onto one (possibly several) models and reporting their performance. In this context, "data that makes a good model" is regarded as "good data."

% To the best of our knowledge, most current studies arbitrarily define their own singular experimental settings and assess data quality by comparing the performance of models trained under these settings. We have observed that the configurations established for training such evaluation models are often set without clear rationale and are not standardized across different studies. Table~\ref{} illustrates the various hyperparameter settings adopted when performing IT using sampled 1K general domain IT data in existing research. As evident, even when training the same model with the same data size, the settings differ across studies.


==> sections/prevs/Section1_241213-1314.tex <==
\section{Introduction}

Instruction Tuning (IT) is widely adopted strategy for enabling a human-interactive use of the knowledge embedded in LLMs \cite{cao2023instruction}. By training with datasets composed of instruction-response pairs, LLM can attain ability to generate appropriate responses to given instructions \cite{dubois2023alpacafarm, zheng2023judging, xu2023wizardlm, conover2023free}.

In implementing IT, data quality is considered a critical factor \cite{lima, liu2024what, treeinst, lu2024instag}. Several research has proven that selectively using high-quality IT data for training leads to better alignment performance than using the entire dataset \cite{chen2024alpagasus, zhao2024long, mekala2024smaller}.

To conduct such research, it's essential to verify the quality of the constructed data. Most studies to date have quantified the quality of IT data by reporting the performance of models trained on it. Under the assumption that "good data makes a good model," the quality of IT data is thus represented by the performance of the models trained on it.

IT는 LLM의 knowledge base를 human-interactive하게 사용할 수 있도록 만드는 매우 효과적인 기술이다 \cite{cao2023instruction}. instruction-response pair로 이루어진 데이터로 학습함으로써, 모델은 주어진 instruction에 대한 적절한 답변을 생성할 수 있게 된다.

In implementing IT, data quality is considered a crucial factor. 다량의 IT데이터가 확보되더라도, 그 데이터를 전부 사용하여 학습하는 것보다 그 중 고품질의 IT를 선별하여 학습하는 것이 더욱 높은 alignment성능을 내는 데 더욱 효과적이라는 것은, 여러 연구들을 통해 밝혀진 바 있다.

이러한 연구들을 수행하는 데 있어서는, 구축된 데이터가 고품질이라는 점을 검증할 필요가 있다. 지금까지 거의 모든 연구들에서는, IT 데이터의 품질을 정량화하기 위해, 해당 데이터로 학습된 모델의 성능을 reporting하는 방법을 사용하고 있다. 즉, under the assumption that "good data makes a good model", 주어진 IT 데이터의 품질은 이를 통해 학습된 모델의 성능으로 represent되고 있다. 

\input{Tables/tb_survey}

이들 대부분은 하나의 실험 세팅을 정의하고, 동일한 실험 세팅 내에서 학습된 모델의 성능을 비교하는 방식을 적용하고 있다. 하지만 우리는, 이러한 연구들에서 검증용 모델 학습을 위한 hyperparameter setting에 대해서 거의 아무런 justification도 이루어지고 있지 않음을 발견하였다.
Table~\ref{tb:survey} illustrates the various hyperparameter settings adopted when performing IT using sampled 1K general domain IT data in existing research. As evident, even when training the same model with the same data size, the settings differ across studies.

In this study, 우리는 이렇게 다른 세팅 하에서 coherent conclusion을 얻어질 수 있는지에 대해 의문을 가진다. In particular, we highlight that the conclusion on the data quality can be reported differently depending on the arbitrarily chosen hyperparameter settings. 이는 보여주고자 하는 목표에 따라서 이후 심각한 confusion을 발생시킬 위험이 있다. For example, even if one reported that A dataset is better than B dataset, the other can also report that B is better than A by training models with different settings.

As a representative case, we consider two datasets for evaluation: LIMA and Alpaca-longest, which is sampled 1K dataset from Alpaca. In \cite{zhao2024long}, it was reported that a model trained on Alpaca-longest outperformed a model trained on LIMA. However, with experiments with LLAMA-2 and Mistral, we demonstrate that LIMA can also be regarded as better than Alpaca-longest, depending on the training setting. 검증용 모델의 hyperparameter가 임의대로 결정되고 있는 현재 연구 기조상, 이러한 confusion은 지금도 발생하고 있는 serious problem이다.

In this study, 우리는 이러한 혼란을 피하기 위해 rigorously performing hyperparameter selection when reporting data quality가 필요함을 밝힌다. 또한, 우리의 discussion을 통해, locally optimal hyperparameter를 찾고, 이러한 세팅 하에서 data quality를 보고할 필요가 있음을 제안한다. 


% We demonstrate how such conclusions can change depending on the hyperparameter selection during the training of the evaluation model, and we draw the community's attention to the ambiguity resulting from these differences.

% Finally, we emphasize the necessity of rigorously performing hyperparameter selection when reporting data quality, and we propose a protocol for more robust and rigorous reporting of experimental results.


% LLM은 remarkable proficiency across a broad spectrum of language understanding and generation tasks, adhering to human instructions with effectiveness and safety. 다양한 분야에서 높은 적응성을 보이며 활발하게 사용되고 있다. 
% 이러한 효과를 얻는 데에는, LLM의 high human-interactive performance가 일조한다고 볼 수 있다. 이러한 capability를 얻기 위해 수행되는 Instruction tuning (IT)는 large language model을 human-interative aligning하기 위해 사용되는 가장 prevalent방법 중 한가지이다. 

% 이를 수행함에 있어서 data quality는 매우 중요한 요소로 여겨진다. 최근 LIMA에서는 1천개의 데이터만으로 high alignment performance를 얻을 수 있음을 보여주고 있으며, alpagasus등의 연구에서는, 다량의 데이터를 사용하는 것보다, 좋은 품질의 데이터만을 선별해서 사용하는 것이 higher performance를 위해 필수적인 요소임을 보여주고 있다. 이러한 연구들에 힘입어, 현재 다수의 연구들은 고품질의 instruction tuning data의 선별이라는 주제를 두고 다양한 방법론들을 시도하고 있다. 

% 이러한 연구들은 under the assumption that "good data makes good model"하에 진행된다. In terms of training data, "good data" is defined as a data that makes "good model". 이에, 대부분의 연구들에서는 검증을 목표로 하는 data가 high quality임을 보여주기 위해, 하나의 모델 (possibly several models)을 학습하고, 이들의 성능을 report하는 방법을 사용한다. 이 경우, "data that makes good model" is regarded as "good data". 

% However, as far as we know, 현재 대부분의 연구들은 자체적인 experimental setting을 한가지 정의해두고, 이 세팅 하에 학습된 모델의 성능을 비교하는 방식으로 데이터의 품질을 가늠하고 있다. 이 상황에서 우리가 발견한 것은, 이러한 검증용 모델을 학습하는 데 있어서 세워지는 세팅이, 별다른 rationale 없이 설정되고 있으며, 심지어 서로 다른 연구들간에 통일되어 있지도 않다는 것이다. Table~\ref{}는, 기존 연구들에서 lima데이터를 사용하여 IT를 수행할 때 도입한 hyperparameter setting을 보여준다. 이를 통해 확인할 수 있듯, 동일한 모델, 동일한 데이터로 학습하는 경우에 있어서도, 세팅은 모두 서로 다르다는 것을 확인할 수 있다.

% 우리는 이러한 방식의 검증을 수행하고 결과를 report를 함에 있어서 주의해야 할 필요가 있음을 밝힌다. 특히, 우리는 어떠한 hyperparameter setting을 선택하는지에 따라서 reporting 결과가 다르게 해석될 수 있음을 밝힌다.
% One may wonder that, coherent한 experimental setting을 정의하고 평가용 모델을 학습했다면, data quality에 대해서 robust한 결론을 내릴 수 있는 것이 아닌지 의문을 가질 수 있다. 하지만 아무리 동일한 세팅을 결정한다 하더라도, 우리가 hyperparameter setting을 임의대로 결정한다면, 데이터 품질에 대한 우리의 결론도 우리의 자의적으로 내릴 수 있다고 말할 수 있다. 

% 우리는 대표적으로 Lima데이터와 Alpaca-longest데이터 두가지를 평가 대상으로 삼는다. \cite{zhao2024long}에서 alpaca-longest로 학습한 모델은 lima로 학습한 모델보다 우월한 성능을 보였음이 report된 바 있다. 우리는 평가용 모델 학습을 위한 hyperparameter selection에 따라서, 이러한 결론이 어떻게 바뀔 수 있는지 보고하며, 이러한 차이에 따른 ambiguity에 대한 community의 관심을 환기한다.

% 우리는 최종적으로, 데이터 품질을 report함에 있어서, hyperparameter 결정을 엄밀하게 수행할 필요가 있음을 밝히며, 보다 robust하고 엄밀한 실험 결과 reporting을 위한 protocol에 대해 제안한다. 


% These studies are conducted under the assumption that "good data makes a good model." In terms of training data, "good data" is defined as data that produces a "good model." Consequently, most studies aim to demonstrate the quality of the data under evaluation by training such data onto one (possibly several) models and reporting their performance. In this context, "data that makes a good model" is regarded as "good data."

% To the best of our knowledge, most current studies arbitrarily define their own singular experimental settings and assess data quality by comparing the performance of models trained under these settings. We have observed that the configurations established for training such evaluation models are often set without clear rationale and are not standardized across different studies. Table~\ref{} illustrates the various hyperparameter settings adopted when performing IT using sampled 1K general domain IT data in existing research. As evident, even when training the same model with the same data size, the settings differ across studies.

% Large Language Models (LLMs) exhibit remarkable proficiency across a broad spectrum of language understanding and generation tasks. Their adaptability and strong human-interactive capability make them valuable across various fields. Instruction Tuning (IT) is one of the most prevalent methods to attain such human-interactive capability. 
% IT involves finetuning LLMs using instruction-response pair data, enabling LLMs to generate appropriate text responses to human instructions.
% It facilitates the alignment of models with human preferences and their knowledge base, enabling the generation of desired outputs in response to various instructions \cite{cao2023instruction}.

% 본인들이 구축한 데이터와 baseline데이터를 LLM에 학습하고, 학습된 모델의 성능을 비교하는 방식의 평가 방법을 적용하였다. 이 경우, 학습된 모델의 성능은 데이터의 품질을 대표한다고 간주된다. These studies mostly  conducted under the assumption that "good data makes a good model." Consequently, most studies aim to demonstrate the quality of the data under evaluation by training such data onto one (possibly several) models and reporting their performance. In this context, "data that makes a good model" is regarded as "good data."

% One might question that coherently applied training setting을 통해 학습했다면, data quality에 대해 robust한 비교가 가능하고, 이에 따라 reliable한 결론을 내릴 수 있는것 아닌가 하며 의문을 가질 수 있다. However, we identify that even with an identical setting, if hyperparameter choices are made arbitrarily, conclusions regarding data quality can also be arbitrarily determined.

==> sections/prevs/Section1_______tex <==
\section{Introduction}

Instruction Tuning데이터가 좋은지 아닌지 판별하기 위해서는 어떻게 해야 할까?
tuning이후 tuning된 모델의 성능을 보는 것이 가장 일반적이고 가장 compelling한 검증 방식일 것이다.

IT 는 활발하게 이루어지고 있다. 

하지만 기존 연구들은 대부분 자의적으로 선택한 hyperparameter setting 한가지 하에서 모든 실험들을 수행한다.

이는 자체적으로 봤을 때는 큰 문제가 없는 것으로 보일 수 있으나, IT를 통해 데이터의 품질을 비교하는 부분에 있어서는 practical challenge가 존재한다. 

이를 보다 명확하게 밝히기 위해서 우리는 다음과 같은 toy experiment를 수행한다.

Instruction tuning (IT)는 large language model을 human-interative aligning하기 위해 사용되는 가장 prevalent방법 중 한가지이다. 이를 수행함에 있어서 data quality는 매우 중요한 요소로 여겨진다. 최근 LIMA에서는 1천개의 데이터만으로 high alignment performance를 얻을 수 있음을 보여주고 있으며, alpagasus등의 연구에서는, 다량의 데이터를 사용하는 것보다, 좋은 품질의 데이터만을 선별해서 사용하는 것이 higher performance를 위해 필수적인 요소임을 보여주고 있다. 

Instruction Tuning데이터가 좋은지 아닌지 판별하기 위해서는 어떻게 해야 할까?

이러한 연구들은 under the assumption that "good data makes good model"하에 진행된다. In terms of training data, "good data" is defined as a data that makes "good model". 이에, 대부분의 연구들에서는 검증을 목표로 하는 data가 high quality임을 보여주기 위해, 하나의 모델 (possibly several models)을 학습하고, 이들의 성능을 report하는 방법을 사용한다. 이 경우, "data that makes good model" is regarded as "good data". 이는 아마 매우 직관적이고 당연한 방법일 것이다.

하지만 우리는 이러한 방식의 검증을 수행하고 결과를 report를 함에 있어서, 우리가 주의해야 할 필요가 있음을 밝힌다. 현재 대부분의 연구들에서는 predefined single training 세팅 내에서 학습된 모델의 성능을 비교하는 방식으로 데이터 품질을 가늠하고 있다. 하지만 우리는 이 경우에, 어떠한 hyperparameter setting을 선택하는지에 따라서 reporting 결과가 다르게 해석될 여지가 있음을 밝힌다.

이러한 위험들을 보다 명확하게 밝히기 위해, 우리는 다음과 같은 toy experiment를 수행했다. 먼저 우리는 alignment tuning을 위하여 설계된 두개의 데이터를 준비하였다. lima와 longest-alpaca. 그리고 우리는 두가지 학습 세팅을 설정하였다. 첫번째는 ...setting이고, 두번째는 ...setting이다. 실험 결과는 어떻게 됐을까? setting1에서는 lima로 학습한 모델의 성능이 좋았으며, setting2에서는 longest-alpaca로 학습한 모델의 성능이 더 좋았다. 

이는 hyperparameter setting이 결과 reporting에 미치는 영향이 생각보다 거대하다는 점을 보여준다. 단순하게 수치의 변동 뿐 아니라, 실험의 결론을 내릴 수 있는 부분까지

기존 연구들은 이러한 차이에 대한 고려가 전혀 이루어지지 않았고, 동일한 세팅 내에서 수행한 실험임을 report하기만 하는 것이 하나의 관례처럼 이루어져 왔다. 이에 만약 우리가 setting1을 사용하기로 결정하기만 하면 우리는 실험 결과에서 lima가 좋은 데이터다 라고 충분히 결론내릴 수 있을 것이다. 물론 만약 setting2를 사용하기로 결정하고, 이를 hyperparameter setting에 명시하기만 한다면 longest가 더 좋은 데이터라고 reporting할 수도 있다.

우리는 여기서 serious deceit이 일어날 여지가 매우 크다고 본다. 이에 우리는 본 연구에서,  instruction tuned model의 성능을 보고함에 있어서 
hyperparamter에 따라 발생할 수 있는 차이를 명확하게 report하고, further study에서도 이러한 부분에 대한 clarity가 필요함을 제안한다. 

